TAG: Task-based Accumulated Gradients for Lifelong learning

When an agent encounters a continual stream of new tasks in the lifelong learning setting, it leverages the knowledge it gained from the earlier tasks to help learn the new tasks better. In such a scenario, identifying an efficient knowledge representation becomes a challenging problem. Most research works propose to either store a subset of examples from the past tasks in a replay buffer, dedicate a separate set of parameters to each task or penalize excessive updates over parameters by introducing a regularization term. While existing methods employ the general task-agnostic stochastic gradient descent update rule, we propose a task-aware optimizer that adapts the learning rate based on the relatedness among tasks. We utilize the directions taken by the parameters during the updates by accumulating the gradients specific to each task. These task-based accumulated gradients act as a knowledge base that is maintained and updated throughout the stream. We empirically show that our proposed adaptive learning rate not only accounts for catastrophic forgetting but also allows positive backward transfer. We also show that our method performs better than several state-of-the-art methods in lifelong learning on complex datasets with a large number of tasks.

==> CoLLAs camera ready/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
% \newcommand{\figleft}{{\em (Left)}}
% \newcommand{\figcenter}{{\em (Center)}}
% \newcommand{\figright}{{\em (Right)}}
% \newcommand{\figtop}{{\em (Top)}}
% \newcommand{\figbottom}{{\em (Bottom)}}
% \newcommand{\captiona}{{\em (a)}}
% \newcommand{\captionb}{{\em (b)}}
% \newcommand{\captionc}{{\em (c)}}
% \newcommand{\captiond}{{\em (d)}}

% % Highlight a newly defined term
% \newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
% \newcommand{\train}{\mathcal{D}}
% \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
% \newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
% \newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
% \newcommand{\pdata}{p_{\rm{data}}}
% % The empirical distribution defined by the training set
% \newcommand{\ptrain}{\hat{p}_{\rm{data}}}
% \newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% % The model distribution
% \newcommand{\pmodel}{p_{\rm{model}}}
% \newcommand{\Pmodel}{P_{\rm{model}}}
% \newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% % Stochastic autoencoder distributions
% \newcommand{\pencode}{p_{\rm{encoder}}}
% \newcommand{\pdecode}{p_{\rm{decoder}}}
% \newcommand{\precons}{p_{\rm{reconstruct}}}

% \newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
% \newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\emp}{\tilde{p}}
% \newcommand{\lr}{\alpha}
% \newcommand{\reg}{\lambda}
% \newcommand{\rect}{\mathrm{rectifier}}
% \newcommand{\softmax}{\mathrm{softmax}}
% \newcommand{\sigmoid}{\sigma}
% \newcommand{\softplus}{\zeta}
% \newcommand{\KL}{D_{\mathrm{KL}}}
% \newcommand{\Var}{\mathrm{Var}}
% \newcommand{\standarderror}{\mathrm{SE}}
% \newcommand{\Cov}{\mathrm{Cov}}
% % Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% % But then they seem to use $L^2$ for vectors throughout the site, and so does
% % wikipedia.
% \newcommand{\normlzero}{L^0}
% \newcommand{\normlone}{L^1}
% \newcommand{\normltwo}{L^2}
% \newcommand{\normlp}{L^p}
% \newcommand{\normmax}{L^\infty}

% \newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

% %%%%% NEW MATH DEFINITIONS %%%%%

% \usepackage{amsmath,amsfonts,bm}

% % Mark sections of captions for referring to divisions of figures
% \newcommand{\figleft}{{\em (Left)}}
% \newcommand{\figcenter}{{\em (Center)}}
% \newcommand{\figright}{{\em (Right)}}
% \newcommand{\figtop}{{\em (Top)}}
% \newcommand{\figbottom}{{\em (Bottom)}}
% \newcommand{\captiona}{{\em (a)}}
% \newcommand{\captionb}{{\em (b)}}
% \newcommand{\captionc}{{\em (c)}}
% \newcommand{\captiond}{{\em (d)}}

% % Highlight a newly defined term
% \newcommand{\newterm}[1]{{\bf #1}}


% % Figure reference, lower-case.
% \def\figref#1{figure~\ref{#1}}
% % Figure reference, capital. For start of sentence
% \def\Figref#1{Figure~\ref{#1}}
% \def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
% \def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% % Section reference, lower-case.
% \def\secref#1{section~\ref{#1}}
% % Section reference, capital.
% \def\Secref#1{Section~\ref{#1}}
% % Reference to two sections.
% \def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% % Reference to three sections.
% \def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% % Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% % Reference to an equation, upper case
% \def\Eqref#1{Equation~\ref{#1}}
% % A raw reference to an equation---avoid using if possible
% \def\plaineqref#1{\ref{#1}}
% % Reference to a chapter, lower-case.
% \def\chapref#1{chapter~\ref{#1}}
% % Reference to an equation, upper case.
% \def\Chapref#1{Chapter~\ref{#1}}
% % Reference to a range of chapters
% \def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% % Reference to an algorithm, lower-case.
% \def\algref#1{algorithm~\ref{#1}}
% % Reference to an algorithm, upper case.
% \def\Algref#1{Algorithm~\ref{#1}}
% \def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
% \def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% % Reference to a part, lower case
% \def\partref#1{part~\ref{#1}}
% % Reference to a part, upper case
% \def\Partref#1{Part~\ref{#1}}
% \def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

% \def\ceil#1{\lceil #1 \rceil}
% \def\floor#1{\lfloor #1 \rfloor}
% \def\1{\bm{1}}
% \newcommand{\train}{\mathcal{D}}
% \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

% \def\eps{{\epsilon}}


% % Random variables
% \def\reta{{\textnormal{$\eta$}}}
% \def\ra{{\textnormal{a}}}
% \def\rb{{\textnormal{b}}}
% \def\rc{{\textnormal{c}}}
% \def\rd{{\textnormal{d}}}
% \def\re{{\textnormal{e}}}
% \def\rf{{\textnormal{f}}}
% \def\rg{{\textnormal{g}}}
% \def\rh{{\textnormal{h}}}
% \def\ri{{\textnormal{i}}}
% \def\rj{{\textnormal{j}}}
% \def\rk{{\textnormal{k}}}
% \def\rl{{\textnormal{l}}}
% % rm is already a command, just don't name any random variables m
% \def\rn{{\textnormal{n}}}
% \def\ro{{\textnormal{o}}}
% \def\rp{{\textnormal{p}}}
% \def\rq{{\textnormal{q}}}
% \def\rr{{\textnormal{r}}}
% \def\rs{{\textnormal{s}}}
% \def\rt{{\textnormal{t}}}
% \def\ru{{\textnormal{u}}}
% \def\rv{{\textnormal{v}}}
% \def\rw{{\textnormal{w}}}
% \def\rx{{\textnormal{x}}}
% \def\ry{{\textnormal{y}}}
% \def\rz{{\textnormal{z}}}

% % Random vectors
% \def\rvepsilon{{\mathbf{\epsilon}}}
% \def\rvtheta{{\mathbf{\theta}}}
% \def\rva{{\mathbf{a}}}
% \def\rvb{{\mathbf{b}}}
% \def\rvc{{\mathbf{c}}}
% \def\rvd{{\mathbf{d}}}
% \def\rve{{\mathbf{e}}}
% \def\rvf{{\mathbf{f}}}
% \def\rvg{{\mathbf{g}}}
% \def\rvh{{\mathbf{h}}}
% \def\rvu{{\mathbf{i}}}
% \def\rvj{{\mathbf{j}}}
% \def\rvk{{\mathbf{k}}}
% \def\rvl{{\mathbf{l}}}
% \def\rvm{{\mathbf{m}}}
% \def\rvn{{\mathbf{n}}}
% \def\rvo{{\mathbf{o}}}
% \def\rvp{{\mathbf{p}}}
% \def\rvq{{\mathbf{q}}}
% \def\rvr{{\mathbf{r}}}
% \def\rvs{{\mathbf{s}}}
% \def\rvt{{\mathbf{t}}}
% \def\rvu{{\mathbf{u}}}
% \def\rvv{{\mathbf{v}}}
% \def\rvw{{\mathbf{w}}}
% \def\rvx{{\mathbf{x}}}
% \def\rvy{{\mathbf{y}}}
% \def\rvz{{\mathbf{z}}}

% % Elements of random vectors
% \def\erva{{\textnormal{a}}}
% \def\ervb{{\textnormal{b}}}
% \def\ervc{{\textnormal{c}}}
% \def\ervd{{\textnormal{d}}}
% \def\erve{{\textnormal{e}}}
% \def\ervf{{\textnormal{f}}}
% \def\ervg{{\textnormal{g}}}
% \def\ervh{{\textnormal{h}}}
% \def\ervi{{\textnormal{i}}}
% \def\ervj{{\textnormal{j}}}
% \def\ervk{{\textnormal{k}}}
% \def\ervl{{\textnormal{l}}}
% \def\ervm{{\textnormal{m}}}
% \def\ervn{{\textnormal{n}}}
% \def\ervo{{\textnormal{o}}}
% \def\ervp{{\textnormal{p}}}
% \def\ervq{{\textnormal{q}}}
% \def\ervr{{\textnormal{r}}}
% \def\ervs{{\textnormal{s}}}
% \def\ervt{{\textnormal{t}}}
% \def\ervu{{\textnormal{u}}}
% \def\ervv{{\textnormal{v}}}
% \def\ervw{{\textnormal{w}}}
% \def\ervx{{\textnormal{x}}}
% \def\ervy{{\textnormal{y}}}
% \def\ervz{{\textnormal{z}}}

% % Random matrices
% \def\rmA{{\mathbf{A}}}
% \def\rmB{{\mathbf{B}}}
% \def\rmC{{\mathbf{C}}}
% \def\rmD{{\mathbf{D}}}
% \def\rmE{{\mathbf{E}}}
% \def\rmF{{\mathbf{F}}}
% \def\rmG{{\mathbf{G}}}
% \def\rmH{{\mathbf{H}}}
% \def\rmI{{\mathbf{I}}}
% \def\rmJ{{\mathbf{J}}}
% \def\rmK{{\mathbf{K}}}
% \def\rmL{{\mathbf{L}}}
% \def\rmM{{\mathbf{M}}}
% \def\rmN{{\mathbf{N}}}
% \def\rmO{{\mathbf{O}}}
% \def\rmP{{\mathbf{P}}}
% \def\rmQ{{\mathbf{Q}}}
% \def\rmR{{\mathbf{R}}}
% \def\rmS{{\mathbf{S}}}
% \def\rmT{{\mathbf{T}}}
% \def\rmU{{\mathbf{U}}}
% \def\rmV{{\mathbf{V}}}
% \def\rmW{{\mathbf{W}}}
% \def\rmX{{\mathbf{X}}}
% \def\rmY{{\mathbf{Y}}}
% \def\rmZ{{\mathbf{Z}}}

% % Elements of random matrices
% \def\ermA{{\textnormal{A}}}
% \def\ermB{{\textnormal{B}}}
% \def\ermC{{\textnormal{C}}}
% \def\ermD{{\textnormal{D}}}
% \def\ermE{{\textnormal{E}}}
% \def\ermF{{\textnormal{F}}}
% \def\ermG{{\textnormal{G}}}
% \def\ermH{{\textnormal{H}}}
% \def\ermI{{\textnormal{I}}}
% \def\ermJ{{\textnormal{J}}}
% \def\ermK{{\textnormal{K}}}
% \def\ermL{{\textnormal{L}}}
% \def\ermM{{\textnormal{M}}}
% \def\ermN{{\textnormal{N}}}
% \def\ermO{{\textnormal{O}}}
% \def\ermP{{\textnormal{P}}}
% \def\ermQ{{\textnormal{Q}}}
% \def\ermR{{\textnormal{R}}}
% \def\ermS{{\textnormal{S}}}
% \def\ermT{{\textnormal{T}}}
% \def\ermU{{\textnormal{U}}}
% \def\ermV{{\textnormal{V}}}
% \def\ermW{{\textnormal{W}}}
% \def\ermX{{\textnormal{X}}}
% \def\ermY{{\textnormal{Y}}}
% \def\ermZ{{\textnormal{Z}}}

% % Vectors
% \def\vzero{{\bm{0}}}
% \def\vone{{\bm{1}}}
% \def\vmu{{\bm{\mu}}}
% \def\vtheta{{\bm{\theta}}}
% \def\va{{\bm{a}}}
% \def\vb{{\bm{b}}}
% \def\vc{{\bm{c}}}
% \def\vd{{\bm{d}}}
% \def\ve{{\bm{e}}}
% \def\vf{{\bm{f}}}
% \def\vg{{\bm{g}}}
% \def\vh{{\bm{h}}}
% \def\vi{{\bm{i}}}
% \def\vj{{\bm{j}}}
% \def\vk{{\bm{k}}}
% \def\vl{{\bm{l}}}
% \def\vm{{\bm{m}}}
% \def\vn{{\bm{n}}}
% \def\vo{{\bm{o}}}
% \def\vp{{\bm{p}}}
% \def\vq{{\bm{q}}}
% \def\vr{{\bm{r}}}
% \def\vs{{\bm{s}}}
% \def\vt{{\bm{t}}}
% \def\vu{{\bm{u}}}
% \def\vv{{\bm{v}}}
% \def\vw{{\bm{w}}}
% \def\vx{{\bm{x}}}
% \def\vy{{\bm{y}}}
% \def\vz{{\bm{z}}}

% % Elements of vectors
% \def\evalpha{{\alpha}}
% \def\evbeta{{\beta}}
% \def\evepsilon{{\epsilon}}
% \def\evlambda{{\lambda}}
% \def\evomega{{\omega}}
% \def\evmu{{\mu}}
% \def\evpsi{{\psi}}
% \def\evsigma{{\sigma}}
% \def\evtheta{{\theta}}
% \def\eva{{a}}
% \def\evb{{b}}
% \def\evc{{c}}
% \def\evd{{d}}
% \def\eve{{e}}
% \def\evf{{f}}
% \def\evg{{g}}
% \def\evh{{h}}
% \def\evi{{i}}
% \def\evj{{j}}
% \def\evk{{k}}
% \def\evl{{l}}
% \def\evm{{m}}
% \def\evn{{n}}
% \def\evo{{o}}
% \def\evp{{p}}
% \def\evq{{q}}
% \def\evr{{r}}
% \def\evs{{s}}
% \def\evt{{t}}
% \def\evu{{u}}
% \def\evv{{v}}
% \def\evw{{w}}
% \def\evx{{x}}
% \def\evy{{y}}
% \def\evz{{z}}

% % Matrix
% \def\mA{{\bm{A}}}
% \def\mB{{\bm{B}}}
% \def\mC{{\bm{C}}}
% \def\mD{{\bm{D}}}
% \def\mE{{\bm{E}}}
% \def\mF{{\bm{F}}}
% \def\mG{{\bm{G}}}
% \def\mH{{\bm{H}}}
% \def\mI{{\bm{I}}}
% \def\mJ{{\bm{J}}}
% \def\mK{{\bm{K}}}
% \def\mL{{\bm{L}}}
% \def\mM{{\bm{M}}}
% \def\mN{{\bm{N}}}
% \def\mO{{\bm{O}}}
% \def\mP{{\bm{P}}}
% \def\mQ{{\bm{Q}}}
% \def\mR{{\bm{R}}}
% \def\mS{{\bm{S}}}
% \def\mT{{\bm{T}}}
% \def\mU{{\bm{U}}}
% \def\mV{{\bm{V}}}
% \def\mW{{\bm{W}}}
% \def\mX{{\bm{X}}}
% \def\mY{{\bm{Y}}}
% \def\mZ{{\bm{Z}}}
% \def\mBeta{{\bm{\beta}}}
% \def\mPhi{{\bm{\Phi}}}
% \def\mLambda{{\bm{\Lambda}}}
% \def\mSigma{{\bm{\Sigma}}}

% % Tensor
% \DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
% \SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
% \newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
% \def\tA{{\tens{A}}}
% \def\tB{{\tens{B}}}
% \def\tC{{\tens{C}}}
% \def\tD{{\tens{D}}}
% \def\tE{{\tens{E}}}
% \def\tF{{\tens{F}}}
% \def\tG{{\tens{G}}}
% \def\tH{{\tens{H}}}
% \def\tI{{\tens{I}}}
% \def\tJ{{\tens{J}}}
% \def\tK{{\tens{K}}}
% \def\tL{{\tens{L}}}
% \def\tM{{\tens{M}}}
% \def\tN{{\tens{N}}}
% \def\tO{{\tens{O}}}
% \def\tP{{\tens{P}}}
% \def\tQ{{\tens{Q}}}
% \def\tR{{\tens{R}}}
% \def\tS{{\tens{S}}}
% \def\tT{{\tens{T}}}
% \def\tU{{\tens{U}}}
% \def\tV{{\tens{V}}}
% \def\tW{{\tens{W}}}
% \def\tX{{\tens{X}}}
% \def\tY{{\tens{Y}}}
% \def\tZ{{\tens{Z}}}


% % Graph
% \def\gA{{\mathcal{A}}}
% \def\gB{{\mathcal{B}}}
% \def\gC{{\mathcal{C}}}
% \def\gD{{\mathcal{D}}}
% \def\gE{{\mathcal{E}}}
% \def\gF{{\mathcal{F}}}
% \def\gG{{\mathcal{G}}}
% \def\gH{{\mathcal{H}}}
% \def\gI{{\mathcal{I}}}
% \def\gJ{{\mathcal{J}}}
% \def\gK{{\mathcal{K}}}
% \def\gL{{\mathcal{L}}}
% \def\gM{{\mathcal{M}}}
% \def\gN{{\mathcal{N}}}
% \def\gO{{\mathcal{O}}}
% \def\gP{{\mathcal{P}}}
% \def\gQ{{\mathcal{Q}}}
% \def\gR{{\mathcal{R}}}
% \def\gS{{\mathcal{S}}}
% \def\gT{{\mathcal{T}}}
% \def\gU{{\mathcal{U}}}
% \def\gV{{\mathcal{V}}}
% \def\gW{{\mathcal{W}}}
% \def\gX{{\mathcal{X}}}
% \def\gY{{\mathcal{Y}}}
% \def\gZ{{\mathcal{Z}}}

% % Sets
% \def\sA{{\mathbb{A}}}
% \def\sB{{\mathbb{B}}}
% \def\sC{{\mathbb{C}}}
% \def\sD{{\mathbb{D}}}
% % Don't use a set called E, because this would be the same as our symbol
% % for expectation.
% \def\sF{{\mathbb{F}}}
% \def\sG{{\mathbb{G}}}
% \def\sH{{\mathbb{H}}}
% \def\sI{{\mathbb{I}}}
% \def\sJ{{\mathbb{J}}}
% \def\sK{{\mathbb{K}}}
% \def\sL{{\mathbb{L}}}
% \def\sM{{\mathbb{M}}}
% \def\sN{{\mathbb{N}}}
% \def\sO{{\mathbb{O}}}
% \def\sP{{\mathbb{P}}}
% \def\sQ{{\mathbb{Q}}}
% \def\sR{{\mathbb{R}}}
% \def\sS{{\mathbb{S}}}
% \def\sT{{\mathbb{T}}}
% \def\sU{{\mathbb{U}}}
% \def\sV{{\mathbb{V}}}
% \def\sW{{\mathbb{W}}}
% \def\sX{{\mathbb{X}}}
% \def\sY{{\mathbb{Y}}}
% \def\sZ{{\mathbb{Z}}}

% % Entries of a matrix
% \def\emLambda{{\Lambda}}
% \def\emA{{A}}
% \def\emB{{B}}
% \def\emC{{C}}
% \def\emD{{D}}
% \def\emE{{E}}
% \def\emF{{F}}
% \def\emG{{G}}
% \def\emH{{H}}
% \def\emI{{I}}
% \def\emJ{{J}}
% \def\emK{{K}}
% \def\emL{{L}}
% \def\emM{{M}}
% \def\emN{{N}}
% \def\emO{{O}}
% \def\emP{{P}}
% \def\emQ{{Q}}
% \def\emR{{R}}
% \def\emS{{S}}
% \def\emT{{T}}
% \def\emU{{U}}
% \def\emV{{V}}
% \def\emW{{W}}
% \def\emX{{X}}
% \def\emY{{Y}}
% \def\emZ{{Z}}
% \def\emSigma{{\Sigma}}

% % entries of a tensor
% % Same font as tensor, without \bm wrapper
% \newcommand{\etens}[1]{\mathsfit{#1}}
% \def\etLambda{{\etens{\Lambda}}}
% \def\etA{{\etens{A}}}
% \def\etB{{\etens{B}}}
% \def\etC{{\etens{C}}}
% \def\etD{{\etens{D}}}
% \def\etE{{\etens{E}}}
% \def\etF{{\etens{F}}}
% \def\etG{{\etens{G}}}
% \def\etH{{\etens{H}}}
% \def\etI{{\etens{I}}}
% \def\etJ{{\etens{J}}}
% \def\etK{{\etens{K}}}
% \def\etL{{\etens{L}}}
% \def\etM{{\etens{M}}}
% \def\etN{{\etens{N}}}
% \def\etO{{\etens{O}}}
% \def\etP{{\etens{P}}}
% \def\etQ{{\etens{Q}}}
% \def\etR{{\etens{R}}}
% \def\etS{{\etens{S}}}
% \def\etT{{\etens{T}}}
% \def\etU{{\etens{U}}}
% \def\etV{{\etens{V}}}
% \def\etW{{\etens{W}}}
% \def\etX{{\etens{X}}}
% \def\etY{{\etens{Y}}}
% \def\etZ{{\etens{Z}}}

% % The true underlying data generating distribution
% \newcommand{\pdata}{p_{\rm{data}}}
% % The empirical distribution defined by the training set
% \newcommand{\ptrain}{\hat{p}_{\rm{data}}}
% \newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% % The model distribution
% \newcommand{\pmodel}{p_{\rm{model}}}
% \newcommand{\Pmodel}{P_{\rm{model}}}
% \newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% % Stochastic autoencoder distributions
% \newcommand{\pencode}{p_{\rm{encoder}}}
% \newcommand{\pdecode}{p_{\rm{decoder}}}
% \newcommand{\precons}{p_{\rm{reconstruct}}}

% \newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
% \newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\emp}{\tilde{p}}
% \newcommand{\lr}{\alpha}
% \newcommand{\reg}{\lambda}
% \newcommand{\rect}{\mathrm{rectifier}}
% \newcommand{\softmax}{\mathrm{softmax}}
% \newcommand{\sigmoid}{\sigma}
% \newcommand{\softplus}{\zeta}
% \newcommand{\KL}{D_{\mathrm{KL}}}
% \newcommand{\Var}{\mathrm{Var}}
% \newcommand{\standarderror}{\mathrm{SE}}
% \newcommand{\Cov}{\mathrm{Cov}}
% % Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% % But then they seem to use $L^2$ for vectors throughout the site, and so does
% % wikipedia.
% \newcommand{\normlzero}{L^0}
% \newcommand{\normlone}{L^1}
% \newcommand{\normltwo}{L^2}
% \newcommand{\normlp}{L^p}
% \newcommand{\normmax}{L^\infty}

% \newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
% \let\ab\allowbreak


==> CoLLAs camera ready/refs.tex <==
@article{caccia2020online,
  title={Online fast adaptation and knowledge accumulation (osaka): a new approach to continual learning},
  author={Caccia, Massimo and Rodriguez, Pau and Ostapenko, Oleksiy and Normandin, Fabrice and Lin, Min and Page-Caccia, Lucas and Laradji, Issam Hadj and Rish, Irina and Lacoste, Alexandre and V{\'a}zquez, David and others},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  year={2020}
}
@inproceedings{yu2020bdd100k,
  title={Bdd100k: A diverse driving dataset for heterogeneous multitask learning},
  author={Yu, Fisher and Chen, Haofeng and Wang, Xin and Xian, Wenqi and Chen, Yingying and Liu, Fangchen and Madhavan, Vashisht and Darrell, Trevor},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={2636--2645},
  year={2020}
}
@article{liu2016recurrent,
  title={Recurrent neural network for text classification with multi-task learning},
  author={Liu, Pengfei and Qiu, Xipeng and Huang, Xuanjing},
  journal={arXiv preprint arXiv:1605.05101},
  year={2016}
}
@article{yao2020speech,
  title={Speech emotion recognition using fusion of three multi-task learning-based classifiers: HSF-DNN, MS-CNN and LLD-RNN},
  author={Yao, Zengwei and Wang, Zihao and Liu, Weihuang and Liu, Yaqian and Pan, Jiahui},
  journal={Speech Communication},
  volume={120},
  pages={11--19},
  year={2020},
  publisher={Elsevier}
}
@inproceedings{liu2019end,
  title={End-to-end multi-task learning with attention},
  author={Liu, Shikun and Johns, Edward and Davison, Andrew J},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1871--1880},
  year={2019}
}
@inproceedings{dong2015multi,
  title={Multi-task learning for multiple language translation},
  author={Dong, Daxiang and Wu, Hua and He, Wei and Yu, Dianhai and Wang, Haifeng},
  booktitle={Proceedings of the 53rd Annual Meeting of the Association for Computational Linguistics and the 7th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
  pages={1723--1732},
  year={2015}
}
@article{zhang2021survey,
  title={A survey on multi-task learning},
  author={Zhang, Yu and Yang, Qiang},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  year={2021},
  publisher={IEEE}
}
@article{ruder2017overview,
  title={An overview of multi-task learning in deep neural networks},
  author={Ruder, Sebastian},
  journal={arXiv preprint arXiv:1706.05098},
  year={2017}
}
@article{caruana1997multitask,
  title={Multitask learning},
  author={Caruana, Rich},
  journal={Machine learning},
  volume={28},
  number={1},
  pages={41--75},
  year={1997},
  publisher={Springer}
}
@article{lydia2019adagrad,
  title={Adagrad—an optimizer for stochastic gradient descent},
  author={Lydia, Agnes and Francis, Sagayaraj},
  journal={Int. J. Inf. Comput. Sci},
  volume={6},
  number={5},
  year={2019}
}
@inproceedings{dogo2018comparative,
  title={A comparative analysis of gradient descent-based optimization algorithms on convolutional neural networks},
  author={Dogo, EM and Afolabi, OJ and Nwulu, NI and Twala, B and Aigbavboa, CO},
  booktitle={2018 International Conference on Computational Techniques, Electronics and Mechanical Systems (CTEMS)},
  pages={92--99},
  year={2018},
  organization={IEEE}
}
@article{mundt2020wholistic,
  title={A wholistic view of continual learning with deep neural networks: Forgotten lessons and the bridge to active and open world learning},
  author={Mundt, Martin and Hong, Yong Won and Pliushch, Iuliia and Ramesh, Visvanathan},
  journal={arXiv preprint arXiv:2009.01797},
  year={2020}
}
@inproceedings{mirzadeh2020dropout,
  title={Dropout as an implicit gating mechanism for continual learning},
  author={Mirzadeh, Seyed Iman and Farajtabar, Mehrdad and Ghasemzadeh, Hassan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={232--233},
  year={2020}
}
@article{french1999catastrophic,
  title={Catastrophic forgetting in connectionist networks},
  author={French, Robert M},
  journal={Trends in cognitive sciences},
  volume={3},
  number={4},
  pages={128--135},
  year={1999},
  publisher={Elsevier}
}
@article{gama2012survey,
  title={A survey on learning from data streams: current and future trends},
  author={Gama, Joao},
  journal={Progress in Artificial Intelligence},
  volume={1},
  number={1},
  pages={45--55},
  year={2012},
  publisher={Springer}
}
@article{bengio1994learning,
  title={Learning long-term dependencies with gradient descent is difficult},
  author={Bengio, Yoshua and Simard, Patrice and Frasconi, Paolo},
  journal={IEEE transactions on neural networks},
  volume={5},
  number={2},
  pages={157--166},
  year={1994},
  publisher={IEEE}
}
@article{steinwart2009fast,
  title={Fast learning from non-iid observations},
  author={Steinwart, Ingo and Christmann, Andreas},
  journal={Advances in neural information processing systems},
  volume={22},
  pages={1768--1776},
  year={2009}
}
@inproceedings{tan2018survey,
  title={A survey on deep transfer learning},
  author={Tan, Chuanqi and Sun, Fuchun and Kong, Tao and Zhang, Wenchang and Yang, Chao and Liu, Chunfang},
  booktitle={International conference on artificial neural networks},
  pages={270--279},
  year={2018},
  organization={Springer}
}
@article{najafabadi2015deep,
  title={Deep learning applications and challenges in big data analytics},
  author={Najafabadi, Maryam M and Villanustre, Flavio and Khoshgoftaar, Taghi M and Seliya, Naeem and Wald, Randall and Muharemagic, Edin},
  journal={Journal of big data},
  volume={2},
  number={1},
  pages={1--21},
  year={2015},
  publisher={SpringerOpen}
}
@article{wang2020gradient,
  title={Gradient vaccine: Investigating and improving multi-task optimization in massively multilingual models},
  author={Wang, Zirui and Tsvetkov, Yulia and Firat, Orhan and Cao, Yuan},
  journal={arXiv preprint arXiv:2010.05874},
  year={2020}
}
@article{guiroy2020towards,
  title={Towards an Unsupervised Method for Model Selection in Few-Shot Learning},
  author={Guiroy, Simon and Verma, Vikas and Pal, Christopher},
  year={2020}
}
@article{saha2021gradient,
  title={Gradient projection memory for continual learning},
  author={Saha, Gobinda and Garg, Isha and Roy, Kaushik},
  journal={arXiv preprint arXiv:2103.09762},
  year={2021}
}
@article{masana2020class,
  title={Class-incremental learning: survey and performance evaluation},
  author={Masana, Marc and Liu, Xialei and Twardowski, Bartlomiej and Menta, Mikel and Bagdanov, Andrew D and van de Weijer, Joost},
  journal={arXiv preprint arXiv:2010.15277},
  year={2020}
}
@article{crawshaw2020multi,
  title={Multi-task learning with deep neural networks: A survey},
  author={Crawshaw, Michael},
  journal={arXiv preprint arXiv:2009.09796},
  year={2020}
}
@article{yu2020gradient,
  title={Gradient surgery for multi-task learning},
  author={Yu, Tianhe and Kumar, Saurabh and Gupta, Abhishek and Levine, Sergey and Hausman, Karol and Finn, Chelsea},
  journal={arXiv preprint arXiv:2001.06782},
  year={2020}
}
@inproceedings{aljundi2017expert,
  title={Expert gate: Lifelong learning with a network of experts},
  author={Aljundi, Rahaf and Chakravarty, Punarjay and Tuytelaars, Tinne},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3366--3375},
  year={2017}
}
@article{li2020adax,
  title={Adax: Adaptive gradient descent with exponential long term memory},
  author={Li, Wenjie and Zhang, Zhaoyang and Wang, Xinjiang and Luo, Ping},
  journal={arXiv preprint arXiv:2004.09740},
  year={2020}
}
@inproceedings{nesterov1983method,
  title={A method for solving the convex programming problem with convergence rate O (1/k\^{} 2)},
  author={Nesterov, Yurii E},
  booktitle={Dokl. akad. nauk Sssr},
  volume={269},
  pages={543--547},
  year={1983}
}
@inproceedings{sutskever2013importance,
  title={On the importance of initialization and momentum in deep learning},
  author={Sutskever, Ilya and Martens, James and Dahl, George and Hinton, Geoffrey},
  booktitle={International conference on machine learning},
  pages={1139--1147},
  year={2013},
  organization={PMLR}
}
@article{polyak1964some,
  title={Some methods of speeding up the convergence of iteration methods},
  author={Polyak, Boris T},
  journal={Ussr computational mathematics and mathematical physics},
  volume={4},
  number={5},
  pages={1--17},
  year={1964},
  publisher={Elsevier}
}
@article{farquhar2019differentially,
  title={Differentially private continual learning},
  author={Farquhar, Sebastian and Gal, Yarin},
  journal={arXiv preprint arXiv:1902.06497},
  year={2019}
}
@article{parisi2019continual,
  title={Continual lifelong learning with neural networks: A review},
  author={Parisi, German I and Kemker, Ronald and Part, Jose L and Kanan, Christopher and Wermter, Stefan},
  journal={Neural Networks},
  volume={113},
  pages={54--71},
  year={2019},
  publisher={Elsevier}
}
@article{van2020brain,
  title={Brain-inspired replay for continual learning with artificial neural networks},
  author={van de Ven, Gido M and Siegelmann, Hava T and Tolias, Andreas S},
  journal={Nature communications},
  volume={11},
  number={1},
  pages={1--14},
  year={2020},
  publisher={Nature Publishing Group}
}
@article{shin2017continual,
  title={Continual learning with deep generative replay},
  author={Shin, Hanul and Lee, Jung Kwon and Kim, Jaehong and Kim, Jiwon},
  journal={arXiv preprint arXiv:1705.08690},
  year={2017}
}
@article{goodfellow2014generative,
  title={Generative adversarial networks},
  author={Goodfellow, Ian J and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1406.2661},
  year={2014}
}
@article{chaudhry2020using,
  title={Using hindsight to anchor past knowledge in continual learning},
  author={Chaudhry, Arslan and Gordo, Albert and Dokania, Puneet K and Torr, Philip and Lopez-Paz, David},
  journal={arXiv preprint arXiv:2002.08165},
  year={2020}
}
@article{HADSELL20201028,
title = "Embracing Change: Continual Learning in Deep Neural Networks",
journal = "Trends in Cognitive Sciences",
volume = "24",
number = "12",
pages = "1028 - 1040",
year = "2020",
issn = "1364-6613",
doi = "https://doi.org/10.1016/j.tics.2020.09.004",
url = "http://www.sciencedirect.com/science/article/pii/S1364661320302199",
author = "Raia Hadsell and Dushyant Rao and Andrei A. Rusu and Razvan Pascanu",
keywords = "artificial intelligence, memory, meta-learning, non-stationary, lifelong"
}
@incollection{MCCLOSKEY1989109,
title = "Catastrophic Interference in Connectionist Networks: The Sequential Learning Problem",
editor = "Gordon H. Bower",
series = "Psychology of Learning and Motivation",
publisher = "Academic Press",
volume = "24",
pages = "109 - 165",
year = "1989",
issn = "0079-7421",
doi = "https://doi.org/10.1016/S0079-7421(08)60536-8",
url = "http://www.sciencedirect.com/science/article/pii/S0079742108605368",
author = "McCloskey, Michael and J. Cohen, Neal",
}
@article{chen2018lifelong,
  title={Lifelong machine learning},
  author={Chen, Zhiyuan and Liu, Bing},
  journal={Synthesis Lectures on Artificial Intelligence and Machine Learning},
  volume={12},
  number={3},
  pages={9--12},
  year={2018},
  chapter={1},
  publisher={Morgan \& Claypool Publishers}
}
@article{bennani2020generalisation,
  title={Generalisation guarantees for continual learning with orthogonal gradient descent},
  author={Bennani, Mehdi Abbana and Sugiyama, Masashi},
  journal={arXiv preprint arXiv:2006.11942},
  year={2020}
}
@article{rusu2016progressive,
  title={Progressive neural networks},
  author={Rusu, Andrei A and Rabinowitz, Neil C and Desjardins, Guillaume and Soyer, Hubert and Kirkpatrick, James and Kavukcuoglu, Koray and Pascanu, Razvan and Hadsell, Raia},
  journal={arXiv preprint arXiv:1606.04671},
  year={2016}
}
@article{riemer2018learning,
  title={Learning to learn without forgetting by maximizing transfer and minimizing interference},
  author={Riemer, Matthew and Cases, Ignacio and Ajemian, Robert and Liu, Miao and Rish, Irina and Tu, Yuhai and Tesauro, Gerald},
  journal={arXiv preprint arXiv:1810.11910},
  year={2018}
}
@inproceedings{chaudhry2018riemannian,
  title={Riemannian walk for incremental learning: Understanding forgetting and intransigence},
  author={Chaudhry, Arslan and Dokania, Puneet K and Ajanthan, Thalaiyasingam and Torr, Philip HS},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={532--547},
  year={2018}
}
@INPROCEEDINGS{323080,
  author={A. {Robins}},
  booktitle={Proceedings 1993 The First New Zealand International Two-Stream Conference on Artificial Neural Networks and Expert Systems}, 
  title={Catastrophic forgetting in neural networks: the role of rehearsal mechanisms}, 
  year={1993},
  volume={},
  number={},
  pages={65-68},
  doi={10.1109/ANNES.1993.323080}}

@inproceedings{imagenet_cvpr09,
        AUTHOR = {Deng, J. and Dong, W. and Socher, R. and Li, L.-J. and Li, K. and Fei-Fei, L.},
        TITLE = {{ImageNet: A Large-Scale Hierarchical Image Database}},
        BOOKTITLE = {CVPR09},
        YEAR = {2009},
        BIBSOURCE = "http://www.image-net.org/papers/imagenet_cvpr09.bib"}
        
@article{xiao2017fashion,
  title={Fashion-mnist: a novel image dataset for benchmarking machine learning algorithms},
  author={Xiao, Han and Rasul, Kashif and Vollgraf, Roland},
  journal={arXiv preprint arXiv:1708.07747},
  year={2017}
}
@techreport{notmnist,
  title={Notmnist dataset},
  author={Bulatov, Yaroslav},
  institution = {Google (Books/OCR)},
  url = {http://yaroslavvb.blogspot.it/2011/09/notmnist-dataset.html},
  year={2011}
}

@article{netzer2011reading,
  title={Reading digits in natural images with unsupervised feature learning},
  author={Netzer, Yuval and Wang, Tao and Coates, Adam and Bissacco, Alessandro and Wu, Bo and Ng, Andrew Y},
  year={2011}
}
@misc{mnist,
  title={The mnist database of handwritten digits},
  author={LeCun, Yann},
  year={1998},
  url={http://yann.lecun.com/exdb/mnist/,}
}

@article{wah2011caltech,
  title={The caltech-ucsd birds-200-2011 dataset},
  author={Wah, Catherine and Branson, Steve and Welinder, Peter and Perona, Pietro and Belongie, Serge},
  year={2011},
  publisher={California Institute of Technology}
}
@inproceedings{vinyals2016matching,
  title={Matching networks for one shot learning},
  author={Vinyals, Oriol and Blundell, Charles and Lillicrap, Timothy and Wierstra, Daan and others},
  booktitle={Advances in neural information processing systems},
  pages={3630--3638},
  year={2016}
}
@article{krizhevsky2009learning,
  title={Learning multiple layers of features from tiny images},
  author={Krizhevsky, Alex and Hinton, Geoffrey and others},
  year={2009},
  publisher={Citeseer}
}
@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}
@article{duchi2011adaptive,
  title={Adaptive subgradient methods for online learning and stochastic optimization.},
  author={Duchi, John and Hazan, Elad and Singer, Yoram},
  journal={Journal of machine learning research},
  volume={12},
  number={7},
  year={2011}
}
@article{li2017convergence,
  title={Convergence analysis of proximal gradient with momentum for nonconvex optimization},
  author={Li, Qunwei and Zhou, Yi and Liang, Yingbin and Varshney, Pramod K},
  journal={arXiv preprint arXiv:1705.04925},
  year={2017}
}
@article{ruder2016overview,
  title={An overview of gradient descent optimization algorithms},
  author={Ruder, Sebastian},
  journal={arXiv preprint arXiv:1609.04747},
  year={2016}
}
@misc{rmsprop,
  title={{Lecture 6.5---RmsProp: Divide the gradient by a running average of its recent magnitude}},
  author={Tieleman, T. and Hinton, G.},
  howpublished={COURSERA: Neural Networks for Machine Learning},
  year={2012}
}
@inproceedings{rebuffi2017icarl,
  title={icarl: Incremental classifier and representation learning},
  author={Rebuffi, Sylvestre-Alvise and Kolesnikov, Alexander and Sperl, Georg and Lampert, Christoph H},
  booktitle={Proceedings of the IEEE conference on Computer Vision and Pattern Recognition},
  pages={2001--2010},
  year={2017}
}
@article{goodfellow2013empirical,
  title={An empirical investigation of catastrophic forgetting in gradient-based neural networks},
  author={Goodfellow, Ian J and Mirza, Mehdi and Xiao, Da and Courville, Aaron and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1312.6211},
  year={2013}
}
@article{shaker2020modular,
  title={Modular-Relatedness for Continual Learning},
  author={Shaker, Ammar and Yu, Shujian and Alesiani, Francesco},
  journal={arXiv preprint arXiv:2011.01272},
  year={2020}
}
@inproceedings{jerfel2019reconciling,
  title={Reconciling meta-learning and continual learning with online mixtures of tasks},
  author={Jerfel, Ghassen and Grant, Erin and Griffiths, Tom and Heller, Katherine A},
  booktitle={Advances in Neural Information Processing Systems},
  pages={9122--9133},
  year={2019}
}
@article{mermillod2013stability,
  title={The stability-plasticity dilemma: Investigating the continuum from catastrophic forgetting to age-limited learning effects},
  author={Mermillod, Martial and Bugaiska, Aur{\'e}lia and Bonin, Patrick},
  journal={Frontiers in psychology},
  volume={4},
  pages={504},
  year={2013},
  publisher={Frontiers}
}

@article{gupta2020maml,
  title={La-MAML: Look-ahead Meta Learning for Continual Learning},
  author={Gupta, Gunshi and Yadav, Karmesh and Paull, Liam},
  journal={arXiv preprint arXiv:2007.13904},
  year={2020}
}
@article{serra2018overcoming,
  title={Overcoming catastrophic forgetting with agemention to the task},
  author={Serra, Joan and Suris, Didac and Miron, Marius and Karatzoglou, Alexandros},
  journal={arXiv preprint arXiv:1801.01423},
  year={2018}
}
@inproceedings{xu2018reinforced,
  title={Reinforced continual learning},
  author={Xu, Ju and Zhu, Zhanxing},
  booktitle={Advances in Neural Information Processing Systems},
  pages={899--908},
  year={2018}
}
@article{li2019learn,
  title={Learn to grow: A continual structure learning framework for overcoming catastrophic forgetting},
  author={Li, Xilai and Zhou, Yingbo and Wu, Tianfu and Socher, Richard and Xiong, Caiming},
  journal={arXiv preprint arXiv:1904.00310},
  year={2019}
}
@article{chen2015net2net,
  title={Net2net: Accelerating learning via knowledge transfer},
  author={Chen, Tianqi and Goodfellow, Ian and Shlens, Jonathon},
  journal={arXiv preprint arXiv:1511.05641},
  year={2015}
}
@article{sodhani2018training,
  title={On training recurrent neural networks for lifelong learning},
  author={Sodhani, Shagun and Chandar, Sarath and Bengio, Yoshua},
  journal={CoRR, abs/1811.07017},
  year={2018}
}
@article{ebrahimi2019uncertainty,
  title={Uncertainty-guided continual learning with bayesian neural networks},
  author={Ebrahimi, Sayna and Elhoseiny, Mohamed and Darrell, Trevor and Rohrbach, Marcus},
  journal={arXiv preprint arXiv:1906.02425},
  year={2019}
}
@inproceedings{triki2017encoder,
  title={Encoder based lifelong learning},
  author={Triki, Amal Rannen and Aljundi, Rahaf and Blaschko, Matthew B and Tuytelaars, Tinne},
  booktitle={ICCV},
  year={2017}
}
@article{li2017learning,
  title={Learning without forgetting},
  author={Li, Zhizhong and Hoiem, Derek},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={40},
  number={12},
  pages={2935--2947},
  year={2017},
  publisher={IEEE}
}

@article{de2019continual,
  title={Continual learning: A comparative study on how to defy forgetting in classification tasks},
  author={De Lange, Matthias and Aljundi, Rahaf and Masana, Marc and Parisot, Sarah and Jia, Xu and Leonardis, Ales and Slabaugh, Gregory and Tuytelaars, Tinne},
  journal={arXiv preprint arXiv:1909.08383},
  volume={2},
  number={6},
  year={2019}
}
@inproceedings{rao2019continual,
  title={Continual unsupervised representation learning},
  author={Rao, Dushyant and Visin, Francesco and Rusu, Andrei and Pascanu, Razvan and Teh, Yee Whye and Hadsell, Raia},
  booktitle={Advances in Neural Information Processing Systems},
  pages={7647--7657},
  year={2019}
}
@article{kumar2012learning,
  title={Learning task grouping and overlap in multi-task learning},
  author={Kumar, Abhishek and Daume III, Hal},
  journal={arXiv preprint arXiv:1206.6417},
  year={2012}
}
@article{yoon2017lifelong,
  title={Lifelong learning with dynamically expandable networks},
  author={Yoon, Jaehong and Yang, Eunho and Lee, Jeongtae and Hwang, Sung Ju},
  journal={arXiv preprint arXiv:1708.01547},
  year={2017}
}
@inproceedings{ruvolo2013ella,
  title={ELLA: An efficient lifelong learning algorithm},
  author={Ruvolo, Paul and Eaton, Eric},
  booktitle={International Conference on Machine Learning},
  pages={507--515},
  year={2013}
}
@article{zhang2017survey,
  title={A survey on multi-task learning},
  author={Zhang, Yu and Yang, Qiang},
  journal={arXiv preprint arXiv:1707.08114},
  year={2017}
}
@article{blundell2015weight,
  title={Weight uncertainty in neural networks},
  author={Blundell, Charles and Cornebise, Julien and Kavukcuoglu, Koray and Wierstra, Daan},
  journal={arXiv preprint arXiv:1505.05424},
  year={2015}
}

@article{adel2019continual,
  title={Continual Learning with Adaptive Weights (CLAW)},
  author={Adel, Tameem and Zhao, Han and Turner, Richard E},
  journal={arXiv preprint arXiv:1911.09514},
  year={2019}
}

@article{zenke2017continual,
  title={Continual learning through synaptic intelligence},
  author={Zenke, Friedemann and Poole, Ben and Ganguli, Surya},
  journal={Proceedings of machine learning research},
  volume={70},
  pages={3987},
  year={2017},
  publisher={Europe PMC Funders}
}

@article{ebrahimi2020adversarial,
  title={Adversarial continual learning},
  author={Ebrahimi, Sayna and Meier, Franziska and Calandra, Roberto and Darrell, Trevor and Rohrbach, Marcus},
  journal={arXiv preprint arXiv:2003.09553},
  year={2020}
}
@article{kirkpatrick2017overcoming,
  title={Overcoming catastrophic forgetting in neural networks},
  author={Kirkpatrick, James and Pascanu, Razvan and Rabinowitz, Neil and Veness, Joel and Desjardins, Guillaume and Rusu, Andrei A and Milan, Kieran and Quan, John and Ramalho, Tiago and Grabska-Barwinska, Agnieszka and others},
  journal={Proceedings of the national academy of sciences},
  volume={114},
  number={13},
  pages={3521--3526},
  year={2017},
  publisher={National Acad Sciences}
}

@inproceedings{nguyen2018variational,
  title = {Variational Continual Learning},
  author = {Nguyen, Cuong V. and Li, Yingzhen and Bui, Thang D. and Turner, Richard E.},
  booktitle = {International Conference on Learning Representations},
  year = {2018}
}

@article{van2019three,
  title={Three scenarios for continual learning},
  author={van de Ven, Gido M and Tolias, Andreas S},
  journal={arXiv preprint arXiv:1904.07734},
  year={2019}
}

@inproceedings{sener2018multi,
  title={Multi-task learning as multi-objective optimization},
  author={Sener, Ozan and Koltun, Vladlen},
  booktitle={Advances in Neural Information Processing Systems},
  pages={527--538},
  year={2018}
}

@inproceedings{farajtabar2020orthogonal,
  title={Orthogonal gradient descent for continual learning},
  author={Farajtabar, Mehrdad and Azizan, Navid and Mott, Alex and Li, Ang},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={3762--3773},
  year={2020},
  organization={PMLR}
}
@article{chen2018closing,
  title={Closing the generalization gap of adaptive gradient methods in training deep neural networks},
  author={Chen, Jinghui and Zhou, Dongruo and Tang, Yiqi and Yang, Ziyan and Gu, Quanquan},
  journal={arXiv preprint arXiv:1806.06763},
  year={2018}
}
@article{keskar2017improving,
  title={Improving generalization performance by switching from adam to sgd},
  author={Keskar, Nitish Shirish and Socher, Richard},
  journal   = {CoRR},
  volume    = {abs/1712.07628},
  year      = {2017},
  url       = {http://arxiv.org/abs/1712.07628},
  archivePrefix = {arXiv},
  eprint    = {1712.07628},
  timestamp = {Mon, 13 Aug 2018 16:48:22 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1712-07628.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{hsu2018re,
  title={Re-evaluating continual learning scenarios: A categorization and case for strong baselines},
  author={Hsu, Yen-Chang and Liu, Yen-Cheng and Ramasamy, Anita and Kira, Zsolt},
  journal={arXiv preprint arXiv:1810.12488},
  year={2018}
}

@article{mirzadeh2020understanding,
  title={Understanding the role of training regimes in continual learning},
  author={Mirzadeh, Seyed Iman and Farajtabar, Mehrdad and Pascanu, Razvan and Ghasemzadeh, Hassan},
  journal={arXiv preprint arXiv:2006.06958},
  year={2020}
}

@article{chaudhry2018efficient,
  title={Efficient lifelong learning with A-GEM},
  author={Chaudhry, Arslan and Ranzato, Marc'Aurelio and Rohrbach, Marcus and Elhoseiny, Mohamed},
  journal={arXiv preprint arXiv:1812.00420},
  year={2018}
}

@article{finn2017model,
  title={Model-agnostic meta-learning for fast adaptation of deep networks},
  author={Finn, Chelsea and Abbeel, Pieter and Levine, Sergey},
  journal={arXiv preprint arXiv:1703.03400},
  year={2017}
}

@article{guiroy2019towards,
  title={Towards understanding generalization in gradient-based meta-learning},
  author={Guiroy, Simon and Verma, Vikas and Pal, Christopher},
  journal={arXiv preprint arXiv:1907.07287},
  year={2019}
}

@inproceedings{aljundi2019online,
  title={Online continual learning with maximal interfered retrieval},
  author={Aljundi, Rahaf and Belilovsky, Eugene and Tuytelaars, Tinne and Charlin, Laurent and Caccia, Massimo and Lin, Min and Page-Caccia, Lucas},
  booktitle={Advances in Neural Information Processing Systems},
  pages={11849--11860},
  year={2019}
}

@article{vitter1985random,
  title={Random sampling with a reservoir},
  author={Vitter, Jeffrey S},
  journal={ACM Transactions on Mathematical Software (TOMS)},
  volume={11},
  number={1},
  pages={37--57},
  year={1985},
  publisher={ACM New York, NY, USA}
}
@article{jin2020gradient,
  title={Gradient Based Memory Editing for Task-Free Continual Learning},
  author={Jin, Xisen and Du, Junyi and Ren, Xiang},
  journal={arXiv preprint arXiv:2006.15294},
  year={2020}
}

@article{chaudhry2019tiny,
  title={On tiny episodic memories in continual learning},
  author={Chaudhry, Arslan and Rohrbach, Marcus and Elhoseiny, Mohamed and Ajanthan, Thalaiyasingam and Dokania, Puneet K and Torr, Philip HS and Ranzato, Marc'Aurelio},
  journal={arXiv preprint arXiv:1902.10486},
  year={2019}
}

@inproceedings{lopez2017gradient,
  title={Gradient episodic memory for continual learning},
  author={Lopez-Paz, David and Ranzato, Marc'Aurelio},
  booktitle={Advances in neural information processing systems},
  pages={6467--6476},
  year={2017}
}
@article{schwarz2018progress,
  title={Progress \& compress: A scalable framework for continual learning},
  author={Schwarz, Jonathan and Luketina, Jelena and Czarnecki, Wojciech M and Grabska-Barwinska, Agnieszka and Teh, Yee Whye and Pascanu, Razvan and Hadsell, Raia},
  journal={arXiv preprint arXiv:1805.06370},
  year={2018}
}
@inproceedings{ahn2019uncertainty,
  title={Uncertainty-based continual learning with adaptive regularization},
  author={Ahn, Hongjoon and Cha, Sungmin and Lee, Donggyu and Moon, Taesup},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4392--4402},
  year={2019}
}

@incollection{Bengio+chapter2007,
author = {Bengio, Yoshua and LeCun, Yann},
booktitle = {Large Scale Kernel Machines},
publisher = {MIT Press},
title = {Scaling Learning Algorithms Towards {AI}},
year = {2007}
}

@article{Hinton06,
author = {Hinton, Geoffrey E. and Osindero, Simon and Teh, Yee Whye},
journal = {Neural Computation},
pages = {1527--1554},
title = {A Fast Learning Algorithm for Deep Belief Nets},
volume = {18},
year = {2006}
}

@book{goodfellow2016deep,
title={Deep learning},
author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron and Bengio, Yoshua},
volume={1},
year={2016},
publisher={MIT Press}
}

==> refs.tex <==
@article{caccia2020online,
  title={Online fast adaptation and knowledge accumulation (osaka): a new approach to continual learning},
  author={Caccia, Massimo and Rodriguez, Pau and Ostapenko, Oleksiy and Normandin, Fabrice and Lin, Min and Page-Caccia, Lucas and Laradji, Issam Hadj and Rish, Irina and Lacoste, Alexandre and V{\'a}zquez, David and others},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  year={2020}
}
@inproceedings{yu2020bdd100k,
  title={Bdd100k: A diverse driving dataset for heterogeneous multitask learning},
  author={Yu, Fisher and Chen, Haofeng and Wang, Xin and Xian, Wenqi and Chen, Yingying and Liu, Fangchen and Madhavan, Vashisht and Darrell, Trevor},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={2636--2645},
  year={2020}
}
@article{liu2016recurrent,
  title={Recurrent neural network for text classification with multi-task learning},
  author={Liu, Pengfei and Qiu, Xipeng and Huang, Xuanjing},
  journal={arXiv preprint arXiv:1605.05101},
  year={2016}
}
@article{yao2020speech,
  title={Speech emotion recognition using fusion of three multi-task learning-based classifiers: HSF-DNN, MS-CNN and LLD-RNN},
  author={Yao, Zengwei and Wang, Zihao and Liu, Weihuang and Liu, Yaqian and Pan, Jiahui},
  journal={Speech Communication},
  volume={120},
  pages={11--19},
  year={2020},
  publisher={Elsevier}
}
@inproceedings{liu2019end,
  title={End-to-end multi-task learning with attention},
  author={Liu, Shikun and Johns, Edward and Davison, Andrew J},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1871--1880},
  year={2019}
}
@inproceedings{dong2015multi,
  title={Multi-task learning for multiple language translation},
  author={Dong, Daxiang and Wu, Hua and He, Wei and Yu, Dianhai and Wang, Haifeng},
  booktitle={Proceedings of the 53rd Annual Meeting of the Association for Computational Linguistics and the 7th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
  pages={1723--1732},
  year={2015}
}
@article{zhang2021survey,
  title={A survey on multi-task learning},
  author={Zhang, Yu and Yang, Qiang},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  year={2021},
  publisher={IEEE}
}
@article{ruder2017overview,
  title={An overview of multi-task learning in deep neural networks},
  author={Ruder, Sebastian},
  journal={arXiv preprint arXiv:1706.05098},
  year={2017}
}
@article{caruana1997multitask,
  title={Multitask learning},
  author={Caruana, Rich},
  journal={Machine learning},
  volume={28},
  number={1},
  pages={41--75},
  year={1997},
  publisher={Springer}
}
@article{lydia2019adagrad,
  title={Adagrad—an optimizer for stochastic gradient descent},
  author={Lydia, Agnes and Francis, Sagayaraj},
  journal={Int. J. Inf. Comput. Sci},
  volume={6},
  number={5},
  year={2019}
}
@inproceedings{dogo2018comparative,
  title={A comparative analysis of gradient descent-based optimization algorithms on convolutional neural networks},
  author={Dogo, EM and Afolabi, OJ and Nwulu, NI and Twala, B and Aigbavboa, CO},
  booktitle={2018 International Conference on Computational Techniques, Electronics and Mechanical Systems (CTEMS)},
  pages={92--99},
  year={2018},
  organization={IEEE}
}
@article{mundt2020wholistic,
  title={A wholistic view of continual learning with deep neural networks: Forgotten lessons and the bridge to active and open world learning},
  author={Mundt, Martin and Hong, Yong Won and Pliushch, Iuliia and Ramesh, Visvanathan},
  journal={arXiv preprint arXiv:2009.01797},
  year={2020}
}
@inproceedings{mirzadeh2020dropout,
  title={Dropout as an implicit gating mechanism for continual learning},
  author={Mirzadeh, Seyed Iman and Farajtabar, Mehrdad and Ghasemzadeh, Hassan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={232--233},
  year={2020}
}
@article{french1999catastrophic,
  title={Catastrophic forgetting in connectionist networks},
  author={French, Robert M},
  journal={Trends in cognitive sciences},
  volume={3},
  number={4},
  pages={128--135},
  year={1999},
  publisher={Elsevier}
}
@article{gama2012survey,
  title={A survey on learning from data streams: current and future trends},
  author={Gama, Joao},
  journal={Progress in Artificial Intelligence},
  volume={1},
  number={1},
  pages={45--55},
  year={2012},
  publisher={Springer}
}
@article{bengio1994learning,
  title={Learning long-term dependencies with gradient descent is difficult},
  author={Bengio, Yoshua and Simard, Patrice and Frasconi, Paolo},
  journal={IEEE transactions on neural networks},
  volume={5},
  number={2},
  pages={157--166},
  year={1994},
  publisher={IEEE}
}
@article{steinwart2009fast,
  title={Fast learning from non-iid observations},
  author={Steinwart, Ingo and Christmann, Andreas},
  journal={Advances in neural information processing systems},
  volume={22},
  pages={1768--1776},
  year={2009}
}
@inproceedings{tan2018survey,
  title={A survey on deep transfer learning},
  author={Tan, Chuanqi and Sun, Fuchun and Kong, Tao and Zhang, Wenchang and Yang, Chao and Liu, Chunfang},
  booktitle={International conference on artificial neural networks},
  pages={270--279},
  year={2018},
  organization={Springer}
}
@article{najafabadi2015deep,
  title={Deep learning applications and challenges in big data analytics},
  author={Najafabadi, Maryam M and Villanustre, Flavio and Khoshgoftaar, Taghi M and Seliya, Naeem and Wald, Randall and Muharemagic, Edin},
  journal={Journal of big data},
  volume={2},
  number={1},
  pages={1--21},
  year={2015},
  publisher={SpringerOpen}
}
@article{wang2020gradient,
  title={Gradient vaccine: Investigating and improving multi-task optimization in massively multilingual models},
  author={Wang, Zirui and Tsvetkov, Yulia and Firat, Orhan and Cao, Yuan},
  journal={arXiv preprint arXiv:2010.05874},
  year={2020}
}
@article{guiroy2020towards,
  title={Towards an Unsupervised Method for Model Selection in Few-Shot Learning},
  author={Guiroy, Simon and Verma, Vikas and Pal, Christopher},
  year={2020}
}
@article{saha2021gradient,
  title={Gradient projection memory for continual learning},
  author={Saha, Gobinda and Garg, Isha and Roy, Kaushik},
  journal={arXiv preprint arXiv:2103.09762},
  year={2021}
}
@article{masana2020class,
  title={Class-incremental learning: survey and performance evaluation},
  author={Masana, Marc and Liu, Xialei and Twardowski, Bartlomiej and Menta, Mikel and Bagdanov, Andrew D and van de Weijer, Joost},
  journal={arXiv preprint arXiv:2010.15277},
  year={2020}
}
@article{crawshaw2020multi,
  title={Multi-task learning with deep neural networks: A survey},
  author={Crawshaw, Michael},
  journal={arXiv preprint arXiv:2009.09796},
  year={2020}
}
@article{yu2020gradient,
  title={Gradient surgery for multi-task learning},
  author={Yu, Tianhe and Kumar, Saurabh and Gupta, Abhishek and Levine, Sergey and Hausman, Karol and Finn, Chelsea},
  journal={arXiv preprint arXiv:2001.06782},
  year={2020}
}
@inproceedings{aljundi2017expert,
  title={Expert gate: Lifelong learning with a network of experts},
  author={Aljundi, Rahaf and Chakravarty, Punarjay and Tuytelaars, Tinne},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3366--3375},
  year={2017}
}
@article{li2020adax,
  title={Adax: Adaptive gradient descent with exponential long term memory},
  author={Li, Wenjie and Zhang, Zhaoyang and Wang, Xinjiang and Luo, Ping},
  journal={arXiv preprint arXiv:2004.09740},
  year={2020}
}
@inproceedings{nesterov1983method,
  title={A method for solving the convex programming problem with convergence rate O (1/k\^{} 2)},
  author={Nesterov, Yurii E},
  booktitle={Dokl. akad. nauk Sssr},
  volume={269},
  pages={543--547},
  year={1983}
}
@inproceedings{sutskever2013importance,
  title={On the importance of initialization and momentum in deep learning},
  author={Sutskever, Ilya and Martens, James and Dahl, George and Hinton, Geoffrey},
  booktitle={International conference on machine learning},
  pages={1139--1147},
  year={2013},
  organization={PMLR}
}
@article{polyak1964some,
  title={Some methods of speeding up the convergence of iteration methods},
  author={Polyak, Boris T},
  journal={Ussr computational mathematics and mathematical physics},
  volume={4},
  number={5},
  pages={1--17},
  year={1964},
  publisher={Elsevier}
}
@article{farquhar2019differentially,
  title={Differentially private continual learning},
  author={Farquhar, Sebastian and Gal, Yarin},
  journal={arXiv preprint arXiv:1902.06497},
  year={2019}
}
@article{parisi2019continual,
  title={Continual lifelong learning with neural networks: A review},
  author={Parisi, German I and Kemker, Ronald and Part, Jose L and Kanan, Christopher and Wermter, Stefan},
  journal={Neural Networks},
  volume={113},
  pages={54--71},
  year={2019},
  publisher={Elsevier}
}
@article{van2020brain,
  title={Brain-inspired replay for continual learning with artificial neural networks},
  author={van de Ven, Gido M and Siegelmann, Hava T and Tolias, Andreas S},
  journal={Nature communications},
  volume={11},
  number={1},
  pages={1--14},
  year={2020},
  publisher={Nature Publishing Group}
}
@article{shin2017continual,
  title={Continual learning with deep generative replay},
  author={Shin, Hanul and Lee, Jung Kwon and Kim, Jaehong and Kim, Jiwon},
  journal={arXiv preprint arXiv:1705.08690},
  year={2017}
}
@article{goodfellow2014generative,
  title={Generative adversarial networks},
  author={Goodfellow, Ian J and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1406.2661},
  year={2014}
}
@article{chaudhry2020using,
  title={Using hindsight to anchor past knowledge in continual learning},
  author={Chaudhry, Arslan and Gordo, Albert and Dokania, Puneet K and Torr, Philip and Lopez-Paz, David},
  journal={arXiv preprint arXiv:2002.08165},
  year={2020}
}
@article{HADSELL20201028,
title = "Embracing Change: Continual Learning in Deep Neural Networks",
journal = "Trends in Cognitive Sciences",
volume = "24",
number = "12",
pages = "1028 - 1040",
year = "2020",
issn = "1364-6613",
doi = "https://doi.org/10.1016/j.tics.2020.09.004",
url = "http://www.sciencedirect.com/science/article/pii/S1364661320302199",
author = "Raia Hadsell and Dushyant Rao and Andrei A. Rusu and Razvan Pascanu",
keywords = "artificial intelligence, memory, meta-learning, non-stationary, lifelong"
}
@incollection{MCCLOSKEY1989109,
title = "Catastrophic Interference in Connectionist Networks: The Sequential Learning Problem",
editor = "Gordon H. Bower",
series = "Psychology of Learning and Motivation",
publisher = "Academic Press",
volume = "24",
pages = "109 - 165",
year = "1989",
issn = "0079-7421",
doi = "https://doi.org/10.1016/S0079-7421(08)60536-8",
url = "http://www.sciencedirect.com/science/article/pii/S0079742108605368",
author = "McCloskey, Michael and J. Cohen, Neal",
}
@article{chen2018lifelong,
  title={Lifelong machine learning},
  author={Chen, Zhiyuan and Liu, Bing},
  journal={Synthesis Lectures on Artificial Intelligence and Machine Learning},
  volume={12},
  number={3},
  pages={9--12},
  year={2018},
  chapter={1},
  publisher={Morgan \& Claypool Publishers}
}
@article{bennani2020generalisation,
  title={Generalisation guarantees for continual learning with orthogonal gradient descent},
  author={Bennani, Mehdi Abbana and Sugiyama, Masashi},
  journal={arXiv preprint arXiv:2006.11942},
  year={2020}
}
@article{rusu2016progressive,
  title={Progressive neural networks},
  author={Rusu, Andrei A and Rabinowitz, Neil C and Desjardins, Guillaume and Soyer, Hubert and Kirkpatrick, James and Kavukcuoglu, Koray and Pascanu, Razvan and Hadsell, Raia},
  journal={arXiv preprint arXiv:1606.04671},
  year={2016}
}
@article{riemer2018learning,
  title={Learning to learn without forgetting by maximizing transfer and minimizing interference},
  author={Riemer, Matthew and Cases, Ignacio and Ajemian, Robert and Liu, Miao and Rish, Irina and Tu, Yuhai and Tesauro, Gerald},
  journal={arXiv preprint arXiv:1810.11910},
  year={2018}
}
@inproceedings{chaudhry2018riemannian,
  title={Riemannian walk for incremental learning: Understanding forgetting and intransigence},
  author={Chaudhry, Arslan and Dokania, Puneet K and Ajanthan, Thalaiyasingam and Torr, Philip HS},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={532--547},
  year={2018}
}
@INPROCEEDINGS{323080,
  author={A. {Robins}},
  booktitle={Proceedings 1993 The First New Zealand International Two-Stream Conference on Artificial Neural Networks and Expert Systems}, 
  title={Catastrophic forgetting in neural networks: the role of rehearsal mechanisms}, 
  year={1993},
  volume={},
  number={},
  pages={65-68},
  doi={10.1109/ANNES.1993.323080}}

@inproceedings{imagenet_cvpr09,
        AUTHOR = {Deng, J. and Dong, W. and Socher, R. and Li, L.-J. and Li, K. and Fei-Fei, L.},
        TITLE = {{ImageNet: A Large-Scale Hierarchical Image Database}},
        BOOKTITLE = {CVPR09},
        YEAR = {2009},
        BIBSOURCE = "http://www.image-net.org/papers/imagenet_cvpr09.bib"}
        
@article{xiao2017fashion,
  title={Fashion-mnist: a novel image dataset for benchmarking machine learning algorithms},
  author={Xiao, Han and Rasul, Kashif and Vollgraf, Roland},
  journal={arXiv preprint arXiv:1708.07747},
  year={2017}
}
@techreport{notmnist,
  title={Notmnist dataset},
  author={Bulatov, Yaroslav},
  institution = {Google (Books/OCR)},
  url = {http://yaroslavvb.blogspot.it/2011/09/notmnist-dataset.html},
  year={2011}
}

@article{netzer2011reading,
  title={Reading digits in natural images with unsupervised feature learning},
  author={Netzer, Yuval and Wang, Tao and Coates, Adam and Bissacco, Alessandro and Wu, Bo and Ng, Andrew Y},
  year={2011}
}
@misc{mnist,
  title={The mnist database of handwritten digits},
  author={LeCun, Yann},
  year={1998},
  url={http://yann.lecun.com/exdb/mnist/,}
}

@article{wah2011caltech,
  title={The caltech-ucsd birds-200-2011 dataset},
  author={Wah, Catherine and Branson, Steve and Welinder, Peter and Perona, Pietro and Belongie, Serge},
  year={2011},
  publisher={California Institute of Technology}
}
@inproceedings{vinyals2016matching,
  title={Matching networks for one shot learning},
  author={Vinyals, Oriol and Blundell, Charles and Lillicrap, Timothy and Wierstra, Daan and others},
  booktitle={Advances in neural information processing systems},
  pages={3630--3638},
  year={2016}
}
@article{krizhevsky2009learning,
  title={Learning multiple layers of features from tiny images},
  author={Krizhevsky, Alex and Hinton, Geoffrey and others},
  year={2009},
  publisher={Citeseer}
}
@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}
@article{duchi2011adaptive,
  title={Adaptive subgradient methods for online learning and stochastic optimization.},
  author={Duchi, John and Hazan, Elad and Singer, Yoram},
  journal={Journal of machine learning research},
  volume={12},
  number={7},
  year={2011}
}
@article{li2017convergence,
  title={Convergence analysis of proximal gradient with momentum for nonconvex optimization},
  author={Li, Qunwei and Zhou, Yi and Liang, Yingbin and Varshney, Pramod K},
  journal={arXiv preprint arXiv:1705.04925},
  year={2017}
}
@article{ruder2016overview,
  title={An overview of gradient descent optimization algorithms},
  author={Ruder, Sebastian},
  journal={arXiv preprint arXiv:1609.04747},
  year={2016}
}
@misc{rmsprop,
  title={{Lecture 6.5---RmsProp: Divide the gradient by a running average of its recent magnitude}},
  author={Tieleman, T. and Hinton, G.},
  howpublished={COURSERA: Neural Networks for Machine Learning},
  year={2012}
}
@inproceedings{rebuffi2017icarl,
  title={icarl: Incremental classifier and representation learning},
  author={Rebuffi, Sylvestre-Alvise and Kolesnikov, Alexander and Sperl, Georg and Lampert, Christoph H},
  booktitle={Proceedings of the IEEE conference on Computer Vision and Pattern Recognition},
  pages={2001--2010},
  year={2017}
}
@article{goodfellow2013empirical,
  title={An empirical investigation of catastrophic forgetting in gradient-based neural networks},
  author={Goodfellow, Ian J and Mirza, Mehdi and Xiao, Da and Courville, Aaron and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1312.6211},
  year={2013}
}
@article{shaker2020modular,
  title={Modular-Relatedness for Continual Learning},
  author={Shaker, Ammar and Yu, Shujian and Alesiani, Francesco},
  journal={arXiv preprint arXiv:2011.01272},
  year={2020}
}
@inproceedings{jerfel2019reconciling,
  title={Reconciling meta-learning and continual learning with online mixtures of tasks},
  author={Jerfel, Ghassen and Grant, Erin and Griffiths, Tom and Heller, Katherine A},
  booktitle={Advances in Neural Information Processing Systems},
  pages={9122--9133},
  year={2019}
}
@article{mermillod2013stability,
  title={The stability-plasticity dilemma: Investigating the continuum from catastrophic forgetting to age-limited learning effects},
  author={Mermillod, Martial and Bugaiska, Aur{\'e}lia and Bonin, Patrick},
  journal={Frontiers in psychology},
  volume={4},
  pages={504},
  year={2013},
  publisher={Frontiers}
}

@article{gupta2020maml,
  title={La-MAML: Look-ahead Meta Learning for Continual Learning},
  author={Gupta, Gunshi and Yadav, Karmesh and Paull, Liam},
  journal={arXiv preprint arXiv:2007.13904},
  year={2020}
}
@article{serra2018overcoming,
  title={Overcoming catastrophic forgetting with agemention to the task},
  author={Serra, Joan and Suris, Didac and Miron, Marius and Karatzoglou, Alexandros},
  journal={arXiv preprint arXiv:1801.01423},
  year={2018}
}
@inproceedings{xu2018reinforced,
  title={Reinforced continual learning},
  author={Xu, Ju and Zhu, Zhanxing},
  booktitle={Advances in Neural Information Processing Systems},
  pages={899--908},
  year={2018}
}
@article{li2019learn,
  title={Learn to grow: A continual structure learning framework for overcoming catastrophic forgetting},
  author={Li, Xilai and Zhou, Yingbo and Wu, Tianfu and Socher, Richard and Xiong, Caiming},
  journal={arXiv preprint arXiv:1904.00310},
  year={2019}
}
@article{chen2015net2net,
  title={Net2net: Accelerating learning via knowledge transfer},
  author={Chen, Tianqi and Goodfellow, Ian and Shlens, Jonathon},
  journal={arXiv preprint arXiv:1511.05641},
  year={2015}
}
@article{sodhani2018training,
  title={On training recurrent neural networks for lifelong learning},
  author={Sodhani, Shagun and Chandar, Sarath and Bengio, Yoshua},
  journal={CoRR, abs/1811.07017},
  year={2018}
}
@article{ebrahimi2019uncertainty,
  title={Uncertainty-guided continual learning with bayesian neural networks},
  author={Ebrahimi, Sayna and Elhoseiny, Mohamed and Darrell, Trevor and Rohrbach, Marcus},
  journal={arXiv preprint arXiv:1906.02425},
  year={2019}
}
@inproceedings{triki2017encoder,
  title={Encoder based lifelong learning},
  author={Triki, Amal Rannen and Aljundi, Rahaf and Blaschko, Matthew B and Tuytelaars, Tinne},
  booktitle={ICCV},
  year={2017}
}
@article{li2017learning,
  title={Learning without forgetting},
  author={Li, Zhizhong and Hoiem, Derek},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={40},
  number={12},
  pages={2935--2947},
  year={2017},
  publisher={IEEE}
}

@article{de2019continual,
  title={Continual learning: A comparative study on how to defy forgetting in classification tasks},
  author={De Lange, Matthias and Aljundi, Rahaf and Masana, Marc and Parisot, Sarah and Jia, Xu and Leonardis, Ales and Slabaugh, Gregory and Tuytelaars, Tinne},
  journal={arXiv preprint arXiv:1909.08383},
  volume={2},
  number={6},
  year={2019}
}
@inproceedings{rao2019continual,
  title={Continual unsupervised representation learning},
  author={Rao, Dushyant and Visin, Francesco and Rusu, Andrei and Pascanu, Razvan and Teh, Yee Whye and Hadsell, Raia},
  booktitle={Advances in Neural Information Processing Systems},
  pages={7647--7657},
  year={2019}
}
@article{kumar2012learning,
  title={Learning task grouping and overlap in multi-task learning},
  author={Kumar, Abhishek and Daume III, Hal},
  journal={arXiv preprint arXiv:1206.6417},
  year={2012}
}
@article{yoon2017lifelong,
  title={Lifelong learning with dynamically expandable networks},
  author={Yoon, Jaehong and Yang, Eunho and Lee, Jeongtae and Hwang, Sung Ju},
  journal={arXiv preprint arXiv:1708.01547},
  year={2017}
}
@inproceedings{ruvolo2013ella,
  title={ELLA: An efficient lifelong learning algorithm},
  author={Ruvolo, Paul and Eaton, Eric},
  booktitle={International Conference on Machine Learning},
  pages={507--515},
  year={2013}
}
@article{zhang2017survey,
  title={A survey on multi-task learning},
  author={Zhang, Yu and Yang, Qiang},
  journal={arXiv preprint arXiv:1707.08114},
  year={2017}
}
@article{blundell2015weight,
  title={Weight uncertainty in neural networks},
  author={Blundell, Charles and Cornebise, Julien and Kavukcuoglu, Koray and Wierstra, Daan},
  journal={arXiv preprint arXiv:1505.05424},
  year={2015}
}

@article{adel2019continual,
  title={Continual Learning with Adaptive Weights (CLAW)},
  author={Adel, Tameem and Zhao, Han and Turner, Richard E},
  journal={arXiv preprint arXiv:1911.09514},
  year={2019}
}

@article{zenke2017continual,
  title={Continual learning through synaptic intelligence},
  author={Zenke, Friedemann and Poole, Ben and Ganguli, Surya},
  journal={Proceedings of machine learning research},
  volume={70},
  pages={3987},
  year={2017},
  publisher={Europe PMC Funders}
}

@article{ebrahimi2020adversarial,
  title={Adversarial continual learning},
  author={Ebrahimi, Sayna and Meier, Franziska and Calandra, Roberto and Darrell, Trevor and Rohrbach, Marcus},
  journal={arXiv preprint arXiv:2003.09553},
  year={2020}
}
@article{kirkpatrick2017overcoming,
  title={Overcoming catastrophic forgetting in neural networks},
  author={Kirkpatrick, James and Pascanu, Razvan and Rabinowitz, Neil and Veness, Joel and Desjardins, Guillaume and Rusu, Andrei A and Milan, Kieran and Quan, John and Ramalho, Tiago and Grabska-Barwinska, Agnieszka and others},
  journal={Proceedings of the national academy of sciences},
  volume={114},
  number={13},
  pages={3521--3526},
  year={2017},
  publisher={National Acad Sciences}
}

@inproceedings{nguyen2018variational,
  title = {Variational Continual Learning},
  author = {Nguyen, Cuong V. and Li, Yingzhen and Bui, Thang D. and Turner, Richard E.},
  booktitle = {International Conference on Learning Representations},
  year = {2018}
}

@article{van2019three,
  title={Three scenarios for continual learning},
  author={van de Ven, Gido M and Tolias, Andreas S},
  journal={arXiv preprint arXiv:1904.07734},
  year={2019}
}

@inproceedings{sener2018multi,
  title={Multi-task learning as multi-objective optimization},
  author={Sener, Ozan and Koltun, Vladlen},
  booktitle={Advances in Neural Information Processing Systems},
  pages={527--538},
  year={2018}
}

@inproceedings{farajtabar2020orthogonal,
  title={Orthogonal gradient descent for continual learning},
  author={Farajtabar, Mehrdad and Azizan, Navid and Mott, Alex and Li, Ang},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={3762--3773},
  year={2020},
  organization={PMLR}
}
@article{chen2018closing,
  title={Closing the generalization gap of adaptive gradient methods in training deep neural networks},
  author={Chen, Jinghui and Zhou, Dongruo and Tang, Yiqi and Yang, Ziyan and Gu, Quanquan},
  journal={arXiv preprint arXiv:1806.06763},
  year={2018}
}
@article{keskar2017improving,
  title={Improving generalization performance by switching from adam to sgd},
  author={Keskar, Nitish Shirish and Socher, Richard},
  journal   = {CoRR},
  volume    = {abs/1712.07628},
  year      = {2017},
  url       = {http://arxiv.org/abs/1712.07628},
  archivePrefix = {arXiv},
  eprint    = {1712.07628},
  timestamp = {Mon, 13 Aug 2018 16:48:22 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1712-07628.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{hsu2018re,
  title={Re-evaluating continual learning scenarios: A categorization and case for strong baselines},
  author={Hsu, Yen-Chang and Liu, Yen-Cheng and Ramasamy, Anita and Kira, Zsolt},
  journal={arXiv preprint arXiv:1810.12488},
  year={2018}
}

@article{mirzadeh2020understanding,
  title={Understanding the role of training regimes in continual learning},
  author={Mirzadeh, Seyed Iman and Farajtabar, Mehrdad and Pascanu, Razvan and Ghasemzadeh, Hassan},
  journal={arXiv preprint arXiv:2006.06958},
  year={2020}
}

@article{chaudhry2018efficient,
  title={Efficient lifelong learning with A-GEM},
  author={Chaudhry, Arslan and Ranzato, Marc'Aurelio and Rohrbach, Marcus and Elhoseiny, Mohamed},
  journal={arXiv preprint arXiv:1812.00420},
  year={2018}
}

@article{finn2017model,
  title={Model-agnostic meta-learning for fast adaptation of deep networks},
  author={Finn, Chelsea and Abbeel, Pieter and Levine, Sergey},
  journal={arXiv preprint arXiv:1703.03400},
  year={2017}
}

@article{guiroy2019towards,
  title={Towards understanding generalization in gradient-based meta-learning},
  author={Guiroy, Simon and Verma, Vikas and Pal, Christopher},
  journal={arXiv preprint arXiv:1907.07287},
  year={2019}
}

@inproceedings{aljundi2019online,
  title={Online continual learning with maximal interfered retrieval},
  author={Aljundi, Rahaf and Belilovsky, Eugene and Tuytelaars, Tinne and Charlin, Laurent and Caccia, Massimo and Lin, Min and Page-Caccia, Lucas},
  booktitle={Advances in Neural Information Processing Systems},
  pages={11849--11860},
  year={2019}
}

@article{vitter1985random,
  title={Random sampling with a reservoir},
  author={Vitter, Jeffrey S},
  journal={ACM Transactions on Mathematical Software (TOMS)},
  volume={11},
  number={1},
  pages={37--57},
  year={1985},
  publisher={ACM New York, NY, USA}
}
@article{jin2020gradient,
  title={Gradient Based Memory Editing for Task-Free Continual Learning},
  author={Jin, Xisen and Du, Junyi and Ren, Xiang},
  journal={arXiv preprint arXiv:2006.15294},
  year={2020}
}

@article{chaudhry2019tiny,
  title={On tiny episodic memories in continual learning},
  author={Chaudhry, Arslan and Rohrbach, Marcus and Elhoseiny, Mohamed and Ajanthan, Thalaiyasingam and Dokania, Puneet K and Torr, Philip HS and Ranzato, Marc'Aurelio},
  journal={arXiv preprint arXiv:1902.10486},
  year={2019}
}

@inproceedings{lopez2017gradient,
  title={Gradient episodic memory for continual learning},
  author={Lopez-Paz, David and Ranzato, Marc'Aurelio},
  booktitle={Advances in neural information processing systems},
  pages={6467--6476},
  year={2017}
}
@article{schwarz2018progress,
  title={Progress \& compress: A scalable framework for continual learning},
  author={Schwarz, Jonathan and Luketina, Jelena and Czarnecki, Wojciech M and Grabska-Barwinska, Agnieszka and Teh, Yee Whye and Pascanu, Razvan and Hadsell, Raia},
  journal={arXiv preprint arXiv:1805.06370},
  year={2018}
}
@inproceedings{ahn2019uncertainty,
  title={Uncertainty-based continual learning with adaptive regularization},
  author={Ahn, Hongjoon and Cha, Sungmin and Lee, Donggyu and Moon, Taesup},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4392--4402},
  year={2019}
}

@incollection{Bengio+chapter2007,
author = {Bengio, Yoshua and LeCun, Yann},
booktitle = {Large Scale Kernel Machines},
publisher = {MIT Press},
title = {Scaling Learning Algorithms Towards {AI}},
year = {2007}
}

@article{Hinton06,
author = {Hinton, Geoffrey E. and Osindero, Simon and Teh, Yee Whye},
journal = {Neural Computation},
pages = {1527--1554},
title = {A Fast Learning Algorithm for Deep Belief Nets},
volume = {18},
year = {2006}
}

@book{goodfellow2016deep,
title={Deep learning},
author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron and Bengio, Yoshua},
volume={1},
year={2016},
publisher={MIT Press}
}
